[CII] halos in ALPINE galaxies: smoking-gun of galactic outflows?

ALMA observations have revealed that many high redshift galaxies are surrounded by extended (10-15 kpc) [CII]-emitting halos which are not predicted by even the most advanced zoom-in simulations. Using a semi-analytical model, in a previous work we suggested that such halos are produced by starburst-driven, catastrophically cooling outflows. Here, we further improve the model and compare its predictions with data from 7 star-forming ($10\lesssim \rm SFR/ M_\odot \rm yr^{-1}<100$) galaxies at z=4-6, observed in the ALPINE survey. We find that (a) detected [CII] halos are a natural by-product of starburst-driven outflows; (b) the outflow mass loading factors are in the range $4\lesssim\eta\lesssim 7$, with higher $\eta$ values for lower-mass, lower-SFR systems, and scale with stellar mass as $\eta \propto M_*^{-0.43}$, consistently with the momentum-driven hypothesis. Our model suggests that outflows are widespread phenomena in high-z galaxies. However, in low-mass systems the halo extended [CII] emission is likely too faint to be detected with the current levels of sensitivity.

==> Outflows and [CII] Halos ALPINE/additional_tex/additional_def.tex <==

\renewcommand{\d}{\mathrm{d}}
\newcommand{\der}[3][]{\frac{\d ^{#1}#2}{\d {#3}^{#1}}}
\newcommand{\pder}[3][]{\frac{\partial ^{#1}#2}{\partial {#3}^{#1}}}
\let\oldnabla\nabla
\renewcommand{\nabla}{\vec{\oldnabla}}
\newcommand{\lap}{\oldnabla^2}

\newcommand{\red}[1]{{{\textcolor{red}{\textbf{#1}}}}}


==> Outflows and [CII] Halos ALPINE/additional_tex/definitions.tex <==

%%%%% AUTHORS - PLACE YOUR OWN COMMANDS HERE %%%%%

% Please keep new commands to a minimum, and use \newcommand not \def to avoid
% overwriting existing commands. Example:
%\newcommand{\pcm}{\,cm$^{-2}$}	% per cm-squared

% quick alias
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand\quotesingle[1]{`{#1}'}
\newcommand\quotes[1]{``{#1}"}
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 


% solar stuff units
\def\msun{{\rm M}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{{\cal D}_{\odot}}
\def\fsun{\xi_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\msunyr{\msun/{\rm yr}}
% units
\def\mum{\mu {\rm m}}
\newcommand{\angstrom}{\mbox{\normalfont\AA}}
\def\cc{\rm cm^{-3}}
\def\kms{\,\rm km\,s^{-1}}
\def\uflux{{\rm erg}\,{\rm s}^{-1} {\rm cm}^{-2} }
% quantities defs
\def\fdust{\xi_{d}}
\def\fesc{f_{\rm esc}}
\def\td{\tau_{sd}}
% additional wrappers for quantities and units
\def\Dsolar{${\cal D}/\dsun$}
\def\Zsolar{$Z/\zsun$}
\def\DDsolar{\left( {{\cal D}\over \dsun} \right)}
\def\ZZsolar{\left( {Z \over \zsun} \right)}

% LINES
\def\S*{$\Sigma_{\rm SFR}$}
\def\Scii{$\Sigma_{\rm CII}$}
\def\Sciimax{$\Sigma_{\rm CII}^{\rm max}$}
\def\CII{\hbox{[C~$\scriptstyle\rm II $]~}}
\def\CIII{\hbox{C~$\scriptstyle\rm III $]~}}
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]~}}

%\def\CII{[CII]~} 
%\def\CIII{CIII]~}
% IONS
\def\HH{\hbox{H$_2$}~} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HeI{\hbox{He~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\CIion{\hbox{C~$\scriptstyle\rm I $~}}
\def\CIIion{\hbox{C~$\scriptstyle\rm II $~}}
\def\CIIIion{\hbox{C~$\scriptstyle\rm III $~}}
\def\CIVion{\hbox{C~$\scriptstyle\rm IV $~}}
\def\CVIion{\hbox{C~$\scriptstyle\rm VI $~}}
% ion variables
\def\nhh{n_{\rm H2}}
\def\nhi{n_{\rm HI}}
\def\nhii{n_{\rm HII}}
\def\fhh{x_{\rm H2}}
\def\fhi{x_{\rm HI}}
\def\fhii{x_{\rm HII}}
% MIX
\def\fd{f^*_{\rm diss}} 
\def\ks{\kappa_{\rm s}}

% COLORS
\def\cyan{\color{cyan}}
\definecolor{apcolor}{HTML}{b3003b}
\definecolor{afcolor}{HTML}{800080}
\definecolor{lvcolor}{HTML}{DF7401}
\definecolor{mdcolor}{HTML}{01abdf} %mahsa and davide
\definecolor{cbcolor}{HTML}{ff0000}
\definecolor{sccolor}{HTML}{cc5500} %stefano
\definecolor{sgcolor}{HTML}{00cc7a}


==> Outflows and [CII] Halos ALPINE/additional_tex/pack.tex <==

% MNRAS is set in Times font. If you don't have this installed (most LaTeX
% installations will be fine) or prefer the old Computer Modern fonts, comment
% out the following line
\usepackage{newtxtext,newtxmath}
% Depending on your LaTeX fonts installation, you might get better results with one of these:
%\usepackage{mathptmx}
%\usepackage{txfonts}

% Use vector fonts, so it zooms properly in on-screen viewing software
% Don't change these lines unless you know what you are doing
\usepackage[T1]{fontenc}
\usepackage{ae,aecompl}

%%%%% AUTHORS - PLACE YOUR OWN PACKAGES HERE %%%%%

% Only include extra packages if you really need them. Common packages are:
\usepackage{graphicx}	% Including figure files

\let\Bbbk\relax         % remove conflict for dual definition
\usepackage{amsmath}	% Advanced maths commands
\usepackage{amssymb}	% Extra maths symbols
\usepackage{comment}
\usepackage{siunitx}
\usepackage{booktabs}


\usepackage{xcolor}

